Deriving Dagger Compactness

Dagger compact structure is a common assumption in the study of physical process theories, but lacks a clear interpretation. Here we derive dagger compactness from more operational axioms on a category. We first characterise the structure in terms of a simple mapping of states to effects which we call a 'state dagger', before deriving this in any category with 'completely mixed' states and a form of purification, as in quantum theory.

==> eptcsdata.tex <==
\providecommand{\firstpage}{181}
\providecommand{\publicationstatus}{Bob Coecke and Mathew Leifer (Eds.):\\ Quantum Physics and Logic 2019 (QPL)\\
EPTCS 318, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.318.11}{10.4204/EPTCS.318.11}}

